Robust Neighbor Discovery in Multi-Hop Multi-Channel Heterogeneous Wireless Networks

An important first step when deploying a wireless ad hoc network is neighbor discovery in which every node attempts to determine the set of nodes it can communicate with in one wireless hop. In the recent years, cognitive radio (CR) technology has gained attention as an attractive approach to alleviate spectrum congestion. A cognitive radio transceiver can operate over a wide range of frequencies, possibly scanning multiple frequency bands. A cognitive radio node can opportunistically utilize unused wireless spectrum without interference from other wireless devices in its vicinity. Due to spatial variations in frequency usage and hardware variations in radio transceivers, different nodes in the network may perceive different subsets of frequencies available to them for communication. This heterogeneity in the available channel sets across the network increases the complexity of solving the neighbor discovery problem in a cognitive radio network. In this work, we design and analyze several randomized algorithms for neighbor discovery in such a (heterogeneous) network under a variety of assumptions (e.g. maximum node degree known or unknown) for both synchronous and asynchronous systems under minimal knowledge. We also show that our randomized algorithms are naturally suited to tolerate unreliable channels and adversarial attacks.

==> discussion.tex <==
\section{Summary and Discussion}
\label{sec:discussion}




In this paper, we have presented several randomized algorithms for neighbor discovery in an \model{} network both for a synchronous and an asynchronous system, and also analyzed their running time.
\Tabref{summary} summarizes the results of the previous two sections.
%%
%% In this section, 
We now discuss two extensions to our 
%% randomized neighbor discovery 
algorithms to enhance their applicability.

\begin{table}[t]
%%
\begin{center}
\caption{A summary of all randomized neighbor discovery algorithms in this work.}
\label{tab:summary}
\fontsize{8}{9}
\selectfont
%%
\begin{tabular}{|c|c|>{\centering\arraybackslash}m{1.75in}|>{\centering\arraybackslash}m{2.0in}|c|} \hline
\multicolumn{3}{|c|}{\textbf{Assumptions}} & \multirow{2}{*}{\textbf{Time Complexity$^\ast$}} & \multirow{2}{*}{\textbf{Section}} \\ \cline{1-3}
\textbf{Synchrony} & \textbf{Start Times} & \textbf{System Parameters} &  & \\ \hline \hline
%%
Synchronous & Same & know an estimate for an upper bound on $\dmaximum$, given by $\destimate$ &  $O\left( \frac{\max( \acsmaximum, \dmaximum )}{\srminimum} \log(\destimate)\log\left( \frac{\nsize}{\epmaximum}\right)\right)$ & 
\ref{sec:identical|degree} \\ \hline
%%
Synchronous & Same &  - & $O( M \log M )$ where 
$M = \frac{16 \max(\acsmaximum, \dmaximum)}{\srminimum}  \ln\left( \frac{\nsize^2}{\epmaximum} \right)$ & \ref{sec:identical|none}  \\ \hline
%%
Synchronous & Different & know an estimate for an upper bound on $\dmaximum$, given by $\destimate$ &  $O\left( \frac{\max( 2\acsmaximum, \destimate )}{\srminimum} \log\left( \frac{\nsize}{\epmaximum}\right)\right)$ &
\ref{sec:different|degree} \\ \hline
%%
Synchronous & Different & - & $O((M + \vmaximum)\log( M + \vmaximum ))$ where $M =  \frac{16 \max(\acsmaximum, \dmaximum_0)}{\srminimum}  \ln\left( 
\frac{\nsize^2}{\epmaximum} \right)$ &  \ref{sec:different|none} \\ \hline
%%
Asynchronous & Different & know an estimate for an upper bound on $\dmaximum$, given by $\destimate$,  and $\drmaximum \leq \frac{1}{7}$ & $O\left(\frac{\flength \max(2\acsmaximum, 3 \destimate) }{\srminimum} \log\left( \frac{\nsize}{\epsilon} \right) \right)$ & \ref{sec:asynchronous|degree} \\ \hline
%%
Asynchronous & Different & $\drmaximum \leq \frac{1}{48 \left\{  \log\left( \frac{\nsize \acsmaximum}{\epmaximum } \right) + \log \left( 1 + \frac{\vmaximum}{\flength} \right)  + 5 \right\}}$ & 
$O\left( \left( M \flength + \vmaximum \right) \log\left( M + \frac{\vmaximum}{\flength} \right) \right)$ where $M = \frac{48 \max(2\acsmaximum, 3 \dmaximum_0)}{\srminimum} \ln\left( \frac{\nsize^2}{\epsilon} \right) + 1$ & 
\ref{sec:asynchronous|none} \\ \hline
%%
\multicolumn{5}{l}{$^\ast$: In the case of variable start times, the time is measured after the last node has started neighbor discovery} \\
%%
\multicolumn{5}{l}{$\nsize$: total number of CR nodes in the network} \\
%%
\multicolumn{3}{l}{$\dmaximum$: maximum degree of a node on a channel} &
\multicolumn{2}{l}{$\dmaximum_0$: smallest power of two greater than or equal to $\dmaximum$} \\
%%
\multicolumn{3}{l}{$\acsmaximum$: size of the largest available channel set} &
\multicolumn{2}{l}{$\srminimum$: minimum span ratio of a link} \\
%%
\multicolumn{5}{l}{$\epmaximum$: maximum error probability (user-specified)} \\
\multicolumn{5}{l}{$\vmaximum$: maximum difference in the start times of two nodes} \\
%%
\multicolumn{3}{l}{$\flength$: length of a frame} &
\multicolumn{2}{l}{$\drmaximum$: maximum drift rate of a local clock} \\
%%
\end{tabular}
%%
\end{center}
%%
\end{table}


\subsection{Handling Diverse Propagation Characteristics}
 
All algorithms described so far have assumed ``one-for-all'' property that if a link from node $v$ to node $u$ exists on some channel then it also exists on all channels that are present in available channel sets of both $u$ and $v$. That may not hold if different channels have very different propagation characteristics.  In  case the ``one-for-all'' property does not hold, we can partition the channels into \emph{bands} such that the subset of  channels within the same band have very similar propagation characteristics. As a result, ``one-for-all'' holds for each band individually. We say that a link can operate in a band if it can operate on some channel in the band. Each link can then be replaced with multiple links, one for each band it can operate in. Link for each band then has to be discovered separately. This modification increases the running time of our algorithms since more links have to be discovered now. The minimum span-ratio in the network now ranges from $\tfrac{1}{S}$ to $\tfrac{\bminimum}{\acsmaximum}$ instead of $\tfrac{1}{\acsmaximum}$ to $1$, where $\bminimum$ is the size of the smallest band (in terms of number of channels). Further the  term ``$\ln\left( \tfrac{\nsize^2}{\epmaximum} \right)$'' in time complexity expressions is replaced with the term ``$\ln\left( \tfrac{N^2 \bsize}{\epmaximum} \right)$'', where $\bsize$ denote the maximum number of bands in which any link can operate.

\subsection{Handling Lossy Channels}


All algorithms described so far have assumed that channels are reliable in the sense that a node fails to receive a message from its neighbor only due to collision. However, in real world, a node may fail to receive a message due
to other reasons as well such as Gaussian noise or transient interference. Let $\fpmaximum$ with $0 \leq \fpmaximum < 1$ denote the probability that a node fails to receive a message
from its neighbor even in the absence of collision. Nodes may not know $\fpmaximum$. With lossy channels, the probability that a link is covered by a time-slot (in \algoref{identical|degree}, \algoref{identical|nodegree}, \algoref{variable|degree} and \algoref{variable|none}) or an \legal{} frame-pair (in \algoref{asynchronous|degree} and \algoref{asynchronous|none})  is now multiplied by a factor of $1 - \fpmaximum$. For example, the probability expression in \lemref{legal|atleast} now becomes 
 $\tfrac{\srminimum (1 - \fpmaximum)}{8\max(2\acsmaximum, 3\destimate)}$. It can be verified that this has the effect of increasing the running time of an algorithm by a factor of $\tfrac{1}{1 - \fpmaximum}$.

\subsection{Tolerating Jamming Attacks}



%% Other extensions

%% \subsection{Asymmetric Communication Graph}
%% \subsection{Directional Antennas}






==> macros.tex <==
% useful mathematics macros

\newcommand{\ang}[2][{}]{{#1\langle} #2 {#1\rangle}}
%% \newcommand{\Ang}[1]{\Big\langle #1 \Big\rangle}
\newcommand{\ceil}[2][{}]{{#1\lceil} #2 {#1\rceil}}
\newcommand{\floor}[2][{}]{{#1\lfloor} #2 {#1\rfloor}}
%% \newcommand{\implies}{\Rightarrow}
 
\newcommand{\myforall}[4][{}]{\ang[#1]{\forall \: #2 : #3 : #4 }}
\newcommand{\myexists}[4][{}]{\ang[#1]{\exists \: #2 : #3 : #4 }}
\newcommand{\mynexists}[4][{}]{\ang[#1]{\nexists \: #2 : #3 : #4 }}

% for formally defining a notion

%% \newcommand{\defined}{\;\;\stackrel{\triangle}{=}\;\;}
\newcommand{\defined}{\;\;\triangleq\;\;}

%% pseudocode symbols

\newcommand{\myif}{\textbf{if}}
\newcommand{\mythen}{\textbf{then}}
\newcommand{\myelse}{\textbf{else}}
\newcommand{\myendif}{\textbf{endif}}
\newcommand{\myor}{\textbf{or}}
\newcommand{\myand}{\textbf{and}}
\newcommand{\mynot}{\textbf{not}}
\newcommand{\myfor}{\textbf{for}}
\newcommand{\myendfor}{\textbf{endfor}}
\newcommand{\mydo}{\textbf{do}}
\newcommand{\mynull}{\textbf{null}}
\newcommand{\myeach}{\textbf{each}}
\newcommand{\mywhile}{\textbf{while}}
\newcommand{\myendwhile}{\textbf{endwhile}}

\newcommand{\false}{\textsf{false}}
\newcommand{\true}{\textsf{true}}

% various references

\newcommand{\chapref}[1]{Chapter~\ref{chap:#1}}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}
\newcommand{\stref}[1]{step~\ref{step:#1}}
\newcommand{\thmref}[1]{Theorem~\ref{thm:#1}}
\newcommand{\lemref}[1]{Lemma~\ref{lem:#1}}
\newcommand{\corref}[1]{Corollary~\ref{cor:#1}}
\newcommand{\defref}[1]{Definition~\ref{def:#1}}
%% \newcommand{\eqref}[1]{(\ref{eq:#1})}
\newcommand{\eqvref}[1]{Equivalence~(\ref{eqv:#1})}
\newcommand{\ineqref}[1]{Inequality~(\ref{ineq:#1})}
\newcommand{\exref}[1]{Example~\ref{ex:#1}}
\newcommand{\propref}[1]{Proposition~\ref{prop:#1}}
\newcommand{\obsref}[1]{Observation~\ref{obs:#1}}


\newcommand{\Chapref}[1]{Chapter~\ref{chap:#1}}
\newcommand{\Secref}[1]{Section~\ref{sec:#1}}
\newcommand{\Figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\Tabref}[1]{Table~\ref{tab:#1}}
\newcommand{\Stref}[1]{Step~\ref{step:#1}}
\newcommand{\Thmref}[1]{Theorem~\ref{thm:#1}}
\newcommand{\Lemref}[1]{Lemma~\ref{lem:#1}}
\newcommand{\Corref}[1]{Corollary~\ref{cor:#1}}
\newcommand{\Defref}[1]{Definition~\ref{def:#1}}
\newcommand{\Eqref}[1]{(\ref{eq:#1})}
\newcommand{\Eqvref}[1]{Equivalence~(\ref{eqv:#1})}
\newcommand{\Ineqref}[1]{Inequality~(\ref{ineq:#1})}
\newcommand{\Exref}[1]{Example~\ref{ex:#1}}
\newcommand{\Propref}[1]{Proposition~\ref{prop:#1}}
\newcommand{\Obsref}[1]{Observation~\ref{obs:#1}}
